Light stringy states

We carefully study the spectrum of open strings localized at the intersections of D6-branes and identify the lowest massive 'twisted' states and their vertex operators, paying particular attention to the signs of the intersection angles. We argue that the masses of the lightest states scale as M^2 ~ \theta M^2_s and can thus be parametrically smaller than the string scale. Relying on previous analyses, we compute scattering amplitudes of massless 'twisted' open strings and study their factorization, confirming the presence of the light massive states as sub-dominant poles in one of the channels.

==> macro.tex <==
%\usepackage{a4}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{lscape}
\usepackage{cite}
\usepackage{epsfig}
\usepackage{multirow}
%\usepackage{psfig}
\usepackage[all]{xy}
\usepackage{amsmath}
%\usepackage{cite}
%\usepackage[dvips]{geometry}
%\usepackage{lscape}


\DeclareMathOperator{\ch}{ch} \DeclareMathOperator{\ck}{c}
\DeclareMathOperator{\dP}{dP} \DeclareMathOperator{\rank}{rank}

%\def\epsfig{\psfig}
\author{}


% draw box with width #1pt and line thickness #2pt
\newcommand{\drawsquare}[2]{\hbox{%
\rule{#2pt}{#1pt}\hskip-#2pt%  left vertical
\rule{#1pt}{#2pt}\hskip-#1pt%  lower horizontal
\rule[#1pt]{#1pt}{#2pt}}\rule[#1pt]{#2pt}{#2pt}\hskip-#2pt%  upper horizontal
\rule{#2pt}{#1pt}}% right vertical
% Young tableaux
\newcommand{\fund}{\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}}%  fund
\newcommand{\Ysymm}{\raisebox{-.5pt}{\drawsquare{6.5}{0.4}}\hskip-0.4pt%
         \raisebox{-.5pt}{\drawsquare{6.5}{0.4}}}%  symmetric second rank
\newcommand{\Yasymm}{\raisebox{-3.5pt}{\drawsquare{6.5}{0.4}}\hskip-6.9pt%
        \raisebox{3pt}{\drawsquare{6.5}{0.4}}}%  antisymmetric second rank
\newcommand{\antifund}{\overline{\fund}}
\newcommand{\bYasymm}{\overline{\Yasymm}}
\newcommand{\bYsymm}{\overline{\Ysymm}}


\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\mbb}{\mathbb}
\newcommand{\ti}{\times}
\newcommand{\half}{\frac{1}{2}}
%\newcommand{\1}{{\bf 1}}
\newcommand{\3}{{\bf 3}}
%\newcommand{\2}{{\bf 2}}
%\newcommand{\24}{{\bf 24}}
%\newcommand{\10}{{\bf 10}}
\newcommand{\4}{{\bf 4}}
\newcommand{\5}{{\bf 5}}
\newcommand{\6}{{\bf 6}}
\newcommand{\8}{{\bf 8}}
\newcommand{\ergo}{$\Rightarrow$}
\newcommand{\ov}{\overline}
\def\IR{\relax{\rm I\kern-.18em R}}
\def\o#1{\overline{#1}}
\def\IP{\relax{\rm I\kern-.18em P}}
%\def\IC{\relax{\rm I\kern-.48em C}}
\def\inbar{\vrule height1.5ex width.4pt depth0pt}
\def\IC{\relax\,\hbox{$\inbar\kern-.3em{\rm C}$}}



\newcommand{\Z}{\mathbb{Z}}


\def\cn{{\cal N}}
\def\cm{{\cal M}}
\def\ca{{\cal A}}
\def\eps{\epsilon}
\def\T{{\bf T}}
\def\P{{\bf P}}
\def\K3{{\bf K3}}
\def\Om{\Omega}
\def\om{\omega}
\def\th{\theta}
\def\Th{\Theta}
\def\G{\Gamma}
%\def\a{\alpha}
\def\b{\beta}
\def\d{\delta}
%\def\i{\iota}
\def\sig{\sigma}
\def\car{{\cal R}}
\def\ov{\overline}
\def\preal{{\rm Re\,}}
\def\pim{{\rm Im\,}}
\def\raw{\rightarrow}
\def\longraw{\longrightarrow}
\def\n2d{\cN_{V^*}^{\otimes 2}}
\def\sCav{\overline{c}_{\av^*}}

\def\End{\mbox{End}}
\def\IC{\mathbb{C}}
%\def\II{\mathbb{I}}
\def\IE{\mathbb{E}}
\def\IQ{\mathbb{Q}}
\def\IR{\mathbb{R}}
\def\IF{\mathbb{F}}
\def\IZ{\mathbb{Z}}
\def\IO{\mathbb{O}}
\def\IP{\mathbb{P}}
\def\IH{\mathbb{H}}
\def\IK{\mathbb{K}}
\def\coker{{\mathop {\rm coker}}}
\def\Hom{{\rm Hom}}
\def\dim{{\rm dim}}
\def\cN{{\mathcal N}}
\def\cM{{\mathcal M}}
\def\cE{{\mathcal E}}
\def\cS{{\mathcal S}}
\def\cO{{\mathcal O}}
\def\cC{{\mathcal C}}
\def\cF{{\mathcal F}}
\def\cP{{\mathcal P}}
\def\cL{{\mathcal L}}
\def\nn{\nonumber}
\def\td{\mbox{td}}
\def\ch{\mbox{ch}}
\def\rk{\mbox{rk}}
\def\ind{\mbox{ind}}
\def\dirac{\slash{\! \! \! \! D}}
\newcommand{\gen}[2]{{\rm span}_{#1}\left\{#2\right\}}
\def\point{\mbox{pt}}
\def\av{\wedge^2 V}
\def\vv{V \otimes V^*}
\def\Tr{{\mathop {\rm Tr}}}
%\def\theequation{\thesection.\arabic{equation}}
\def\to{\rightarrow}
\def\sC{\bar{c}_U}
\def\im{\mathop {\rm im}}
\def\sym{{\rm Sym}}
\newcommand{\mat}[1]{\left( \matrix{#1} \right)}
\newcommand{\smat}[1]{{\scriptsize \mat{#1}}}
\newcommand{\tmat}[1]{{\tiny \mat{#1}}}
\def\II{{\rlap{1} \hskip 1.6pt \hbox{1}}}
%\newarrow{DotsTo}....>
%\newarrow{DDTo}{}{dash}{}{dash}>
\def\ol{\overline}
\def\navd{\cN_{\av^*}}

